Numerical investigation of fracture behaviour of polyurethane adhesives under the influence of moisture

Polyurethane adhesives are extensively used in manufacturing of the lightweight components. These adhesives are hygroscopic in nature causing the material to degrade their mechanical properties due to ageing under environmental conditions. Polyurethane adhesive shows non-linear rate-dependent behaviour due to viscoelastic properties and assumes nearly incompressible deformation. Finite-strain viscoelastic model is formulated based on the continuum rheological model by combining spring and Maxwell elements in parallel. Nearly incompressible property is considered by decomposing the mechanical free energy into volumetric and isochoric parts. This work focuses on the investigation of the influence of moisture on the fracture behaviour. Phase-field damage model proved to be an efficient method to investigate the fracture behaviour. Therefore, the finite-strain viscoelastic material model is coupled with the phase-field model to investigate fracture behaviour. Material is assumed to be isotropic, therefore the total mechanical energy is considered for bulk degradation. Experiments are conducted on the samples aged for different humid conditions to understand tear strength. These test results are used to identify the phase-field damage material parameters from numerical investigation.

==> phasefield/100RH_KVSZ.tex <==
% GNUPLOT: LaTeX picture with Postscript
\begingroup
\large
  \makeatletter
  \providecommand\color[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package color not loaded in conjunction with
      terminal option `colourtext'%
    }{See the gnuplot documentation for explanation.%
    }{Either use 'blacktext' in gnuplot or load the package
      color.sty in LaTeX.}%
    \renewcommand\color[2][]{}%
  }%
  \providecommand\includegraphics[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package graphicx or graphics not loaded%
    }{See the gnuplot documentation for explanation.%
    }{The gnuplot epslatex terminal needs graphicx.sty or graphics.sty.}%
    \renewcommand\includegraphics[2][]{}%
  }%
  \providecommand\rotatebox[2]{#2}%
  \@ifundefined{ifGPcolor}{%
    \newif\ifGPcolor
    \GPcolortrue
  }{}%
  \@ifundefined{ifGPblacktext}{%
    \newif\ifGPblacktext
    \GPblacktextfalse
  }{}%
  % define a \g@addto@macro without @ in the name:
  \let\gplgaddtomacro\g@addto@macro
  % define empty templates for all commands taking text:
  \gdef\gplbacktext{}%
  \gdef\gplfronttext{}%
  \makeatother
  \ifGPblacktext
    % no textcolor at all
    \def\colorrgb#1{}%
    \def\colorgray#1{}%
  \else
    % gray or color?
    \ifGPcolor
      \def\colorrgb#1{\color[rgb]{#1}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color[rgb]{1,0,0}}%
      \expandafter\def\csname LT1\endcsname{\color[rgb]{0,1,0}}%
      \expandafter\def\csname LT2\endcsname{\color[rgb]{0,0,1}}%
      \expandafter\def\csname LT3\endcsname{\color[rgb]{1,0,1}}%
      \expandafter\def\csname LT4\endcsname{\color[rgb]{0,1,1}}%
      \expandafter\def\csname LT5\endcsname{\color[rgb]{1,1,0}}%
      \expandafter\def\csname LT6\endcsname{\color[rgb]{0,0,0}}%
      \expandafter\def\csname LT7\endcsname{\color[rgb]{1,0.3,0}}%
      \expandafter\def\csname LT8\endcsname{\color[rgb]{0.5,0.5,0.5}}%
    \else
      % gray
      \def\colorrgb#1{\color{black}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color{black}}%
      \expandafter\def\csname LT1\endcsname{\color{black}}%
      \expandafter\def\csname LT2\endcsname{\color{black}}%
      \expandafter\def\csname LT3\endcsname{\color{black}}%
      \expandafter\def\csname LT4\endcsname{\color{black}}%
      \expandafter\def\csname LT5\endcsname{\color{black}}%
      \expandafter\def\csname LT6\endcsname{\color{black}}%
      \expandafter\def\csname LT7\endcsname{\color{black}}%
      \expandafter\def\csname LT8\endcsname{\color{black}}%
    \fi
  \fi
  \setlength{\unitlength}{0.0500bp}%
  \begin{picture}(7200.00,5040.00)%
    \gplgaddtomacro\gplbacktext{%
      \csname LTb\endcsname%
      \put(682,704){\makebox(0,0)[r]{\strut{} 0}}%
      \put(682,1518){\makebox(0,0)[r]{\strut{} 5}}%
      \put(682,2332){\makebox(0,0)[r]{\strut{} 10}}%
      \put(682,3147){\makebox(0,0)[r]{\strut{} 15}}%
      \put(682,3961){\makebox(0,0)[r]{\strut{} 20}}%
      \put(682,4775){\makebox(0,0)[r]{\strut{} 25}}%
      \put(814,484){\makebox(0,0){\strut{} 0}}%
      \put(1413,484){\makebox(0,0){\strut{} 5}}%
      \put(2012,484){\makebox(0,0){\strut{} 10}}%
      \put(2611,484){\makebox(0,0){\strut{} 15}}%
      \put(3210,484){\makebox(0,0){\strut{} 20}}%
      \put(3809,484){\makebox(0,0){\strut{} 25}}%
      \put(4407,484){\makebox(0,0){\strut{} 30}}%
      \put(5006,484){\makebox(0,0){\strut{} 35}}%
      \put(5605,484){\makebox(0,0){\strut{} 40}}%
      \put(6204,484){\makebox(0,0){\strut{} 45}}%
      \put(6803,484){\makebox(0,0){\strut{} 50}}%
      \put(176,2739){\rotatebox{-270}{\makebox(0,0){\strut{}Force $\left[\rm N\right]$}}}%
      \put(4072,154){\makebox(0,0){\strut{}Time $\left[\rm s\right]$}}%
    }%
    \gplgaddtomacro\gplfronttext{%
      \csname LTb\endcsname%
      \put(3718,4514){\makebox(0,0)[r]{\strut{}Standard deviation}}%
      \csname LTb\endcsname%
      \put(3718,4118){\makebox(0,0)[r]{\strut{}100$\%$ r.H. Experiment}}%
      \csname LTb\endcsname%
      \put(3718,3722){\makebox(0,0)[r]{\strut{}100$\%$ r.H. Simulation}}%
    }%
    \gplgaddtomacro\gplbacktext{%
      \csname LTb\endcsname%
      \put(682,704){\makebox(0,0)[r]{\strut{} 0}}%
      \put(682,1518){\makebox(0,0)[r]{\strut{} 5}}%
      \put(682,2332){\makebox(0,0)[r]{\strut{} 10}}%
      \put(682,3147){\makebox(0,0)[r]{\strut{} 15}}%
      \put(682,3961){\makebox(0,0)[r]{\strut{} 20}}%
      \put(682,4775){\makebox(0,0)[r]{\strut{} 25}}%
      \put(814,484){\makebox(0,0){\strut{} 0}}%
      \put(1413,484){\makebox(0,0){\strut{} 5}}%
      \put(2012,484){\makebox(0,0){\strut{} 10}}%
      \put(2611,484){\makebox(0,0){\strut{} 15}}%
      \put(3210,484){\makebox(0,0){\strut{} 20}}%
      \put(3809,484){\makebox(0,0){\strut{} 25}}%
      \put(4407,484){\makebox(0,0){\strut{} 30}}%
      \put(5006,484){\makebox(0,0){\strut{} 35}}%
      \put(5605,484){\makebox(0,0){\strut{} 40}}%
      \put(6204,484){\makebox(0,0){\strut{} 45}}%
      \put(6803,484){\makebox(0,0){\strut{} 50}}%
      \put(176,2739){\rotatebox{-270}{\makebox(0,0){\strut{}Force $\left[\rm N\right]$}}}%
      \put(4072,154){\makebox(0,0){\strut{}Time $\left[\rm s\right]$}}%
    }%
    \gplgaddtomacro\gplfronttext{%
      \csname LTb\endcsname%
      \put(3718,4514){\makebox(0,0)[r]{\strut{}Standard deviation}}%
      \csname LTb\endcsname%
      \put(3718,4118){\makebox(0,0)[r]{\strut{}100$\%$ r.H. Experiment}}%
      \csname LTb\endcsname%
      \put(3718,3722){\makebox(0,0)[r]{\strut{}100$\%$ r.H. Simulation}}%
    }%
    \gplbacktext
    \put(0,0){\includegraphics{phasefield/100RH_KVSZ}}%
    \gplfronttext
  \end{picture}%
\endgroup


==> phasefield/29RH_KVS.tex <==
% GNUPLOT: LaTeX picture with Postscript
\begingroup
  \makeatletter
  \providecommand\color[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package color not loaded in conjunction with
      terminal option `colourtext'%
    }{See the gnuplot documentation for explanation.%
    }{Either use 'blacktext' in gnuplot or load the package
      color.sty in LaTeX.}%
    \renewcommand\color[2][]{}%
  }%
  \providecommand\includegraphics[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package graphicx or graphics not loaded%
    }{See the gnuplot documentation for explanation.%
    }{The gnuplot epslatex terminal needs graphicx.sty or graphics.sty.}%
    \renewcommand\includegraphics[2][]{}%
  }%
  \providecommand\rotatebox[2]{#2}%
  \@ifundefined{ifGPcolor}{%
    \newif\ifGPcolor
    \GPcolortrue
  }{}%
  \@ifundefined{ifGPblacktext}{%
    \newif\ifGPblacktext
    \GPblacktextfalse
  }{}%
  % define a \g@addto@macro without @ in the name:
  \let\gplgaddtomacro\g@addto@macro
  % define empty templates for all commands taking text:
  \gdef\gplbacktext{}%
  \gdef\gplfronttext{}%
  \makeatother
  \ifGPblacktext
    % no textcolor at all
    \def\colorrgb#1{}%
    \def\colorgray#1{}%
  \else
    % gray or color?
    \ifGPcolor
      \def\colorrgb#1{\color[rgb]{#1}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color[rgb]{1,0,0}}%
      \expandafter\def\csname LT1\endcsname{\color[rgb]{0,1,0}}%
      \expandafter\def\csname LT2\endcsname{\color[rgb]{0,0,1}}%
      \expandafter\def\csname LT3\endcsname{\color[rgb]{1,0,1}}%
      \expandafter\def\csname LT4\endcsname{\color[rgb]{0,1,1}}%
      \expandafter\def\csname LT5\endcsname{\color[rgb]{1,1,0}}%
      \expandafter\def\csname LT6\endcsname{\color[rgb]{0,0,0}}%
      \expandafter\def\csname LT7\endcsname{\color[rgb]{1,0.3,0}}%
      \expandafter\def\csname LT8\endcsname{\color[rgb]{0.5,0.5,0.5}}%
    \else
      % gray
      \def\colorrgb#1{\color{black}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color{black}}%
      \expandafter\def\csname LT1\endcsname{\color{black}}%
      \expandafter\def\csname LT2\endcsname{\color{black}}%
      \expandafter\def\csname LT3\endcsname{\color{black}}%
      \expandafter\def\csname LT4\endcsname{\color{black}}%
      \expandafter\def\csname LT5\endcsname{\color{black}}%
      \expandafter\def\csname LT6\endcsname{\color{black}}%
      \expandafter\def\csname LT7\endcsname{\color{black}}%
      \expandafter\def\csname LT8\endcsname{\color{black}}%
    \fi
  \fi
  \setlength{\unitlength}{0.0500bp}%
  \begin{picture}(7200.00,5040.00)%
    \gplgaddtomacro\gplbacktext{%
      \csname LTb\endcsname%
      \put(682,704){\makebox(0,0)[r]{\strut{} 0}}%
      \put(682,1518){\makebox(0,0)[r]{\strut{} 5}}%
      \put(682,2332){\makebox(0,0)[r]{\strut{} 10}}%
      \put(682,3147){\makebox(0,0)[r]{\strut{} 15}}%
      \put(682,3961){\makebox(0,0)[r]{\strut{} 20}}%
      \put(682,4775){\makebox(0,0)[r]{\strut{} 25}}%
      \put(814,484){\makebox(0,0){\strut{} 0}}%
      \put(1479,484){\makebox(0,0){\strut{} 1}}%
      \put(2145,484){\makebox(0,0){\strut{} 2}}%
      \put(2810,484){\makebox(0,0){\strut{} 3}}%
      \put(3476,484){\makebox(0,0){\strut{} 4}}%
      \put(4141,484){\makebox(0,0){\strut{} 5}}%
      \put(4807,484){\makebox(0,0){\strut{} 6}}%
      \put(5472,484){\makebox(0,0){\strut{} 7}}%
      \put(6138,484){\makebox(0,0){\strut{} 8}}%
      \put(6803,484){\makebox(0,0){\strut{} 9}}%
      \put(176,2739){\rotatebox{-270}{\makebox(0,0){\strut{}Force $\left[\rm N\right]$}}}%
      \put(4072,154){\makebox(0,0){\strut{}Displacemenet $\left[\rm mm\right]$}}%
    }%
    \gplgaddtomacro\gplfronttext{%
      \csname LTb\endcsname%
      \put(3586,4602){\makebox(0,0)[r]{\strut{}Standard deviation}}%
      \csname LTb\endcsname%
      \put(3586,4382){\makebox(0,0)[r]{\strut{}29$\%$ r.H. Experiment}}%
      \csname LTb\endcsname%
      \put(3586,4162){\makebox(0,0)[r]{\strut{}29$\%$ r.H. Simlation}}%
    }%
    \gplgaddtomacro\gplbacktext{%
      \csname LTb\endcsname%
      \put(682,704){\makebox(0,0)[r]{\strut{} 0}}%
      \put(682,1518){\makebox(0,0)[r]{\strut{} 5}}%
      \put(682,2332){\makebox(0,0)[r]{\strut{} 10}}%
      \put(682,3147){\makebox(0,0)[r]{\strut{} 15}}%
      \put(682,3961){\makebox(0,0)[r]{\strut{} 20}}%
      \put(682,4775){\makebox(0,0)[r]{\strut{} 25}}%
      \put(814,484){\makebox(0,0){\strut{} 0}}%
      \put(1479,484){\makebox(0,0){\strut{} 1}}%
      \put(2145,484){\makebox(0,0){\strut{} 2}}%
      \put(2810,484){\makebox(0,0){\strut{} 3}}%
      \put(3476,484){\makebox(0,0){\strut{} 4}}%
      \put(4141,484){\makebox(0,0){\strut{} 5}}%
      \put(4807,484){\makebox(0,0){\strut{} 6}}%
      \put(5472,484){\makebox(0,0){\strut{} 7}}%
      \put(6138,484){\makebox(0,0){\strut{} 8}}%
      \put(6803,484){\makebox(0,0){\strut{} 9}}%
      \put(176,2739){\rotatebox{-270}{\makebox(0,0){\strut{}Force $\left[\rm N\right]$}}}%
      \put(4072,154){\makebox(0,0){\strut{}Displacemenet $\left[\rm mm\right]$}}%
    }%
    \gplgaddtomacro\gplfronttext{%
      \csname LTb\endcsname%
      \put(3586,4602){\makebox(0,0)[r]{\strut{}Standard deviation}}%
      \csname LTb\endcsname%
      \put(3586,4382){\makebox(0,0)[r]{\strut{}29$\%$ r.H. Experiment}}%
      \csname LTb\endcsname%
      \put(3586,4162){\makebox(0,0)[r]{\strut{}29$\%$ r.H. Simlation}}%
    }%
    \gplbacktext
    \put(0,0){\includegraphics{29RH_KVS}}%
    \gplfronttext
  \end{picture}%
\endgroup


==> phasefield/29RH_KVSZ.tex <==
% GNUPLOT: LaTeX picture with Postscript
\begingroup
\large
  \makeatletter
  \providecommand\color[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package color not loaded in conjunction with
      terminal option `colourtext'%
    }{See the gnuplot documentation for explanation.%
    }{Either use 'blacktext' in gnuplot or load the package
      color.sty in LaTeX.}%
    \renewcommand\color[2][]{}%
  }%
  \providecommand\includegraphics[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package graphicx or graphics not loaded%
    }{See the gnuplot documentation for explanation.%
    }{The gnuplot epslatex terminal needs graphicx.sty or graphics.sty.}%
    \renewcommand\includegraphics[2][]{}%
  }%
  \providecommand\rotatebox[2]{#2}%
  \@ifundefined{ifGPcolor}{%
    \newif\ifGPcolor
    \GPcolortrue
  }{}%
  \@ifundefined{ifGPblacktext}{%
    \newif\ifGPblacktext
    \GPblacktextfalse
  }{}%
  % define a \g@addto@macro without @ in the name:
  \let\gplgaddtomacro\g@addto@macro
  % define empty templates for all commands taking text:
  \gdef\gplbacktext{}%
  \gdef\gplfronttext{}%
  \makeatother
  \ifGPblacktext
    % no textcolor at all
    \def\colorrgb#1{}%
    \def\colorgray#1{}%
  \else
    % gray or color?
    \ifGPcolor
      \def\colorrgb#1{\color[rgb]{#1}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color[rgb]{1,0,0}}%
      \expandafter\def\csname LT1\endcsname{\color[rgb]{0,1,0}}%
      \expandafter\def\csname LT2\endcsname{\color[rgb]{0,0,1}}%
      \expandafter\def\csname LT3\endcsname{\color[rgb]{1,0,1}}%
      \expandafter\def\csname LT4\endcsname{\color[rgb]{0,1,1}}%
      \expandafter\def\csname LT5\endcsname{\color[rgb]{1,1,0}}%
      \expandafter\def\csname LT6\endcsname{\color[rgb]{0,0,0}}%
      \expandafter\def\csname LT7\endcsname{\color[rgb]{1,0.3,0}}%
      \expandafter\def\csname LT8\endcsname{\color[rgb]{0.5,0.5,0.5}}%
    \else
      % gray
      \def\colorrgb#1{\color{black}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color{black}}%
      \expandafter\def\csname LT1\endcsname{\color{black}}%
      \expandafter\def\csname LT2\endcsname{\color{black}}%
      \expandafter\def\csname LT3\endcsname{\color{black}}%
      \expandafter\def\csname LT4\endcsname{\color{black}}%
      \expandafter\def\csname LT5\endcsname{\color{black}}%
      \expandafter\def\csname LT6\endcsname{\color{black}}%
      \expandafter\def\csname LT7\endcsname{\color{black}}%
      \expandafter\def\csname LT8\endcsname{\color{black}}%
    \fi
  \fi
  \setlength{\unitlength}{0.0500bp}%
  \begin{picture}(7200.00,5040.00)%
    \gplgaddtomacro\gplbacktext{%
      \csname LTb\endcsname%
      \put(682,704){\makebox(0,0)[r]{\strut{} 0}}%
      \put(682,1518){\makebox(0,0)[r]{\strut{} 5}}%
      \put(682,2332){\makebox(0,0)[r]{\strut{} 10}}%
      \put(682,3147){\makebox(0,0)[r]{\strut{} 15}}%
      \put(682,3961){\makebox(0,0)[r]{\strut{} 20}}%
      \put(682,4775){\makebox(0,0)[r]{\strut{} 25}}%
      \put(814,484){\makebox(0,0){\strut{} 0}}%
      \put(1413,484){\makebox(0,0){\strut{} 5}}%
      \put(2012,484){\makebox(0,0){\strut{} 10}}%
      \put(2611,484){\makebox(0,0){\strut{} 15}}%
      \put(3210,484){\makebox(0,0){\strut{} 20}}%
      \put(3809,484){\makebox(0,0){\strut{} 25}}%
      \put(4407,484){\makebox(0,0){\strut{} 30}}%
      \put(5006,484){\makebox(0,0){\strut{} 35}}%
      \put(5605,484){\makebox(0,0){\strut{} 40}}%
      \put(6204,484){\makebox(0,0){\strut{} 45}}%
      \put(6803,484){\makebox(0,0){\strut{} 50}}%
      \put(176,2739){\rotatebox{-270}{\makebox(0,0){\strut{}Force $\left[\rm N\right]$}}}%
      \put(4072,154){\makebox(0,0){\strut{}Time $\left[\rm s\right]$}}%
    }%
    \gplgaddtomacro\gplfronttext{%
      \csname LTb\endcsname%
      \put(3586,4514){\makebox(0,0)[r]{\strut{}Standard deviation}}%
      \csname LTb\endcsname%
      \put(3586,4118){\makebox(0,0)[r]{\strut{}29$\%$ r.H. Experiment}}%
      \csname LTb\endcsname%
      \put(3586,3722){\makebox(0,0)[r]{\strut{}29$\%$ r.H. Simulation}}%
    }%
    \gplgaddtomacro\gplbacktext{%
      \csname LTb\endcsname%
      \put(682,704){\makebox(0,0)[r]{\strut{} 0}}%
      \put(682,1518){\makebox(0,0)[r]{\strut{} 5}}%
      \put(682,2332){\makebox(0,0)[r]{\strut{} 10}}%
      \put(682,3147){\makebox(0,0)[r]{\strut{} 15}}%
      \put(682,3961){\makebox(0,0)[r]{\strut{} 20}}%
      \put(682,4775){\makebox(0,0)[r]{\strut{} 25}}%
      \put(814,484){\makebox(0,0){\strut{} 0}}%
      \put(1413,484){\makebox(0,0){\strut{} 5}}%
      \put(2012,484){\makebox(0,0){\strut{} 10}}%
      \put(2611,484){\makebox(0,0){\strut{} 15}}%
      \put(3210,484){\makebox(0,0){\strut{} 20}}%
      \put(3809,484){\makebox(0,0){\strut{} 25}}%
      \put(4407,484){\makebox(0,0){\strut{} 30}}%
      \put(5006,484){\makebox(0,0){\strut{} 35}}%
      \put(5605,484){\makebox(0,0){\strut{} 40}}%
      \put(6204,484){\makebox(0,0){\strut{} 45}}%
      \put(6803,484){\makebox(0,0){\strut{} 50}}%
      \put(176,2739){\rotatebox{-270}{\makebox(0,0){\strut{}Force $\left[\rm N\right]$}}}%
      \put(4072,154){\makebox(0,0){\strut{}Time $\left[\rm s\right]$}}%
    }%
    \gplgaddtomacro\gplfronttext{%
      \csname LTb\endcsname%
      \put(3586,4514){\makebox(0,0)[r]{\strut{}Standard deviation}}%
      \csname LTb\endcsname%
      \put(3586,4118){\makebox(0,0)[r]{\strut{}29$\%$ r.H. Experiment}}%
      \csname LTb\endcsname%
      \put(3586,3722){\makebox(0,0)[r]{\strut{}29$\%$ r.H. Simulation}}%
    }%
    \gplbacktext
    \put(0,0){\includegraphics{phasefield/29RH_KVSZ}}%
    \gplfronttext
  \end{picture}%
\endgroup


==> phasefield/67RH_KVSZ.tex <==
% GNUPLOT: LaTeX picture with Postscript
\begingroup
\large
  \makeatletter
  \providecommand\color[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package color not loaded in conjunction with
      terminal option `colourtext'%
    }{See the gnuplot documentation for explanation.%
    }{Either use 'blacktext' in gnuplot or load the package
      color.sty in LaTeX.}%
    \renewcommand\color[2][]{}%
  }%
  \providecommand\includegraphics[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package graphicx or graphics not loaded%
    }{See the gnuplot documentation for explanation.%
    }{The gnuplot epslatex terminal needs graphicx.sty or graphics.sty.}%
    \renewcommand\includegraphics[2][]{}%
  }%
  \providecommand\rotatebox[2]{#2}%
  \@ifundefined{ifGPcolor}{%
    \newif\ifGPcolor
    \GPcolortrue
  }{}%
  \@ifundefined{ifGPblacktext}{%
    \newif\ifGPblacktext
    \GPblacktextfalse
  }{}%
  % define a \g@addto@macro without @ in the name:
  \let\gplgaddtomacro\g@addto@macro
  % define empty templates for all commands taking text:
  \gdef\gplbacktext{}%
  \gdef\gplfronttext{}%
  \makeatother
  \ifGPblacktext
    % no textcolor at all
    \def\colorrgb#1{}%
    \def\colorgray#1{}%
  \else
    % gray or color?
    \ifGPcolor
      \def\colorrgb#1{\color[rgb]{#1}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color[rgb]{1,0,0}}%
      \expandafter\def\csname LT1\endcsname{\color[rgb]{0,1,0}}%
      \expandafter\def\csname LT2\endcsname{\color[rgb]{0,0,1}}%
      \expandafter\def\csname LT3\endcsname{\color[rgb]{1,0,1}}%
      \expandafter\def\csname LT4\endcsname{\color[rgb]{0,1,1}}%
      \expandafter\def\csname LT5\endcsname{\color[rgb]{1,1,0}}%
      \expandafter\def\csname LT6\endcsname{\color[rgb]{0,0,0}}%
      \expandafter\def\csname LT7\endcsname{\color[rgb]{1,0.3,0}}%
      \expandafter\def\csname LT8\endcsname{\color[rgb]{0.5,0.5,0.5}}%
    \else
      % gray
      \def\colorrgb#1{\color{black}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color{black}}%
      \expandafter\def\csname LT1\endcsname{\color{black}}%
      \expandafter\def\csname LT2\endcsname{\color{black}}%
      \expandafter\def\csname LT3\endcsname{\color{black}}%
      \expandafter\def\csname LT4\endcsname{\color{black}}%
      \expandafter\def\csname LT5\endcsname{\color{black}}%
      \expandafter\def\csname LT6\endcsname{\color{black}}%
      \expandafter\def\csname LT7\endcsname{\color{black}}%
      \expandafter\def\csname LT8\endcsname{\color{black}}%
    \fi
  \fi
  \setlength{\unitlength}{0.0500bp}%
  \begin{picture}(7200.00,5040.00)%
    \gplgaddtomacro\gplbacktext{%
      \csname LTb\endcsname%
      \put(682,704){\makebox(0,0)[r]{\strut{} 0}}%
      \put(682,1518){\makebox(0,0)[r]{\strut{} 5}}%
      \put(682,2332){\makebox(0,0)[r]{\strut{} 10}}%
      \put(682,3147){\makebox(0,0)[r]{\strut{} 15}}%
      \put(682,3961){\makebox(0,0)[r]{\strut{} 20}}%
      \put(682,4775){\makebox(0,0)[r]{\strut{} 25}}%
      \put(814,484){\makebox(0,0){\strut{} 0}}%
      \put(2012,484){\makebox(0,0){\strut{} 10}}%
      \put(3210,484){\makebox(0,0){\strut{} 20}}%
      \put(4407,484){\makebox(0,0){\strut{} 30}}%
      \put(5605,484){\makebox(0,0){\strut{} 40}}%
      \put(6803,484){\makebox(0,0){\strut{} 50}}%
      \put(176,2739){\rotatebox{-270}{\makebox(0,0){\strut{}Force $\left[\rm N\right]$}}}%
      \put(4072,154){\makebox(0,0){\strut{}Time $\left[\rm s\right]$}}%
    }%
    \gplgaddtomacro\gplfronttext{%
      \csname LTb\endcsname%
      \put(3586,4514){\makebox(0,0)[r]{\strut{}Standard deviation}}%
      \csname LTb\endcsname%
      \put(3586,4118){\makebox(0,0)[r]{\strut{}67$\%$ r.H. Experiment}}%
      \csname LTb\endcsname%
      \put(3586,3722){\makebox(0,0)[r]{\strut{}67$\%$ r.H. Simulation}}%
    }%
    \gplgaddtomacro\gplbacktext{%
      \csname LTb\endcsname%
      \put(682,704){\makebox(0,0)[r]{\strut{} 0}}%
      \put(682,1518){\makebox(0,0)[r]{\strut{} 5}}%
      \put(682,2332){\makebox(0,0)[r]{\strut{} 10}}%
      \put(682,3147){\makebox(0,0)[r]{\strut{} 15}}%
      \put(682,3961){\makebox(0,0)[r]{\strut{} 20}}%
      \put(682,4775){\makebox(0,0)[r]{\strut{} 25}}%
      \put(814,484){\makebox(0,0){\strut{} 0}}%
      \put(2012,484){\makebox(0,0){\strut{} 10}}%
      \put(3210,484){\makebox(0,0){\strut{} 20}}%
      \put(4407,484){\makebox(0,0){\strut{} 30}}%
      \put(5605,484){\makebox(0,0){\strut{} 40}}%
      \put(6803,484){\makebox(0,0){\strut{} 50}}%
      \put(176,2739){\rotatebox{-270}{\makebox(0,0){\strut{}Force $\left[\rm N\right]$}}}%
      \put(4072,154){\makebox(0,0){\strut{}Time $\left[\rm s\right]$}}%
    }%
    \gplgaddtomacro\gplfronttext{%
      \csname LTb\endcsname%
      \put(3586,4514){\makebox(0,0)[r]{\strut{}Standard deviation}}%
      \csname LTb\endcsname%
      \put(3586,4118){\makebox(0,0)[r]{\strut{}67$\%$ r.H. Experiment}}%
      \csname LTb\endcsname%
      \put(3586,3722){\makebox(0,0)[r]{\strut{}67$\%$ r.H. Simulation}}%
    }%
    \gplbacktext
    \put(0,0){\includegraphics{phasefield/67RH_KVSZ}}%
    \gplfronttext
  \end{picture}%
\endgroup


==> phasefield/crack2.tex <==
% GNUPLOT: LaTeX picture with Postscript
\begingroup
\large
  \makeatletter
  \providecommand\color[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package color not loaded in conjunction with
      terminal option `colourtext'%
    }{See the gnuplot documentation for explanation.%
    }{Either use 'blacktext' in gnuplot or load the package
      color.sty in LaTeX.}%
    \renewcommand\color[2][]{}%
  }%
  \providecommand\includegraphics[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package graphicx or graphics not loaded%
    }{See the gnuplot documentation for explanation.%
    }{The gnuplot epslatex terminal needs graphicx.sty or graphics.sty.}%
    \renewcommand\includegraphics[2][]{}%
  }%
  \providecommand\rotatebox[2]{#2}%
  \@ifundefined{ifGPcolor}{%
    \newif\ifGPcolor
    \GPcolortrue
  }{}%
  \@ifundefined{ifGPblacktext}{%
    \newif\ifGPblacktext
    \GPblacktextfalse
  }{}%
  % define a \g@addto@macro without @ in the name:
  \let\gplgaddtomacro\g@addto@macro
  % define empty templates for all commands taking text:
  \gdef\gplbacktext{}%
  \gdef\gplfronttext{}%
  \makeatother
  \ifGPblacktext
    % no textcolor at all
    \def\colorrgb#1{}%
    \def\colorgray#1{}%
  \else
    % gray or color?
    \ifGPcolor
      \def\colorrgb#1{\color[rgb]{#1}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color[rgb]{1,0,0}}%
      \expandafter\def\csname LT1\endcsname{\color[rgb]{0,1,0}}%
      \expandafter\def\csname LT2\endcsname{\color[rgb]{0,0,1}}%
      \expandafter\def\csname LT3\endcsname{\color[rgb]{1,0,1}}%
      \expandafter\def\csname LT4\endcsname{\color[rgb]{0,1,1}}%
      \expandafter\def\csname LT5\endcsname{\color[rgb]{1,1,0}}%
      \expandafter\def\csname LT6\endcsname{\color[rgb]{0,0,0}}%
      \expandafter\def\csname LT7\endcsname{\color[rgb]{1,0.3,0}}%
      \expandafter\def\csname LT8\endcsname{\color[rgb]{0.5,0.5,0.5}}%
    \else
      % gray
      \def\colorrgb#1{\color{black}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color{black}}%
      \expandafter\def\csname LT1\endcsname{\color{black}}%
      \expandafter\def\csname LT2\endcsname{\color{black}}%
      \expandafter\def\csname LT3\endcsname{\color{black}}%
      \expandafter\def\csname LT4\endcsname{\color{black}}%
      \expandafter\def\csname LT5\endcsname{\color{black}}%
      \expandafter\def\csname LT6\endcsname{\color{black}}%
      \expandafter\def\csname LT7\endcsname{\color{black}}%
      \expandafter\def\csname LT8\endcsname{\color{black}}%
    \fi
  \fi
  \setlength{\unitlength}{0.0500bp}%
  \begin{picture}(7200.00,5040.00)%
    \gplgaddtomacro\gplbacktext{%
      \csname LTb\endcsname%
      \put(682,704){\makebox(0,0)[r]{\strut{} 0}}%
      \put(682,1518){\makebox(0,0)[r]{\strut{} 5}}%
      \put(682,2332){\makebox(0,0)[r]{\strut{} 10}}%
      \put(682,3147){\makebox(0,0)[r]{\strut{} 15}}%
      \put(682,3961){\makebox(0,0)[r]{\strut{} 20}}%
      \put(682,4775){\makebox(0,0)[r]{\strut{} 25}}%
      \put(814,484){\makebox(0,0){\strut{} 0}}%
      \put(1479,484){\makebox(0,0){\strut{} 5}}%
      \put(2145,484){\makebox(0,0){\strut{} 10}}%
      \put(2810,484){\makebox(0,0){\strut{} 15}}%
      \put(3476,484){\makebox(0,0){\strut{} 20}}%
      \put(4141,484){\makebox(0,0){\strut{} 25}}%
      \put(4807,484){\makebox(0,0){\strut{} 30}}%
      \put(5472,484){\makebox(0,0){\strut{} 35}}%
      \put(6138,484){\makebox(0,0){\strut{} 40}}%
      \put(6803,484){\makebox(0,0){\strut{} 45}}%
      \put(176,2739){\rotatebox{-270}{\makebox(0,0){\strut{}Force $\left[\rm N\right]$}}}%
      \put(4072,154){\makebox(0,0){\strut{}Time $\left[\rm s\right]$}}%
    }%
    \gplgaddtomacro\gplfronttext{%
      \csname LTb\endcsname%
      \put(3322,4514){\makebox(0,0)[r]{\strut{}Standard deviation}}%
      \csname LTb\endcsname%
      \put(3322,4118){\makebox(0,0)[r]{\strut{}Experiment}}%
      \csname LTb\endcsname%
      \put(3322,3722){\makebox(0,0)[r]{\strut{}Simulation}}%
    }%
    \gplbacktext
    \put(0,0){\includegraphics{phasefield/crack2}}%
    \gplfronttext
  \end{picture}%
\endgroup

